Cosmic Histories of Stars, Gas, Heavy Elements, and Dust

We present a set of coupled equations that relate the stellar, gaseous, chemical, and radiation constituents of the universe averaged over the whole galaxy population. Using as input the available data from quasar absorption-line surveys, optical imaging and redshift surveys, and the COBE DIRBE and FIRAS extragalactic infrared background measurements, we obtain solutions for the cosmic histories of stars, interstellar gas, heavy elements, dust, and radiation from stars and dust in galaxies. Our solutions reproduce remarkably well a wide variety of observations that were not used as input, including the integrated background light from galaxy counts, the optical and near-infrared emissivities from galaxy surveys, the local infrared emissivities from the IRAS survey, the mean abundance of heavy elements from surveys of damped Lyman-alpha systems, and the global star formation rates from H$\alpha$ surveys and submillimeter observations. The solutions presented here suggest that the process of galaxy formation appears to have undergone an early period of substantial inflow to assemble interstellar gas at $z\gtrsim3$, a subsequent period of intense star formation and chemical enrichment at $1\lesssim z\lesssim3$, and a recent period of rapid decline in the gas content, star formation rate, optical stellar emissivity, and infrared dust emission at $z\lesssim1$. [abridged version]

==> apj2col.tex <==
%
% apjtwo.tex
%
 \catcode`@=11
 \newskip\ttglue

 \font\twelverm=cmr12
 \font\eightrm=cmr8   \font\sixrm=cmr6
 \font\eighti=cmmi8   \font\sixi=cmmi6
 \font\eightsy=cmsy8  \font\sixsy=cmsy6
 \font\eightbf=cmbx8  \font\sixbf=cmbx6
 \font\eighttt=cmtt8
 \font\eightit=cmti8
 \font\eightsl=cmsl8

 \def\rm{\fam0\tenrm}%
 \textfont0=\tenrm \scriptfont0=\sevenrm \scriptscriptfont0=\fiverm
 \textfont1=\teni  \scriptfont1=\seveni  \scriptscriptfont1=\fivei
 \textfont2=\tensy \scriptfont2=\sevensy \scriptscriptfont2=\fivesy
 \textfont3=\tenex \scriptfont3=\tenex   \scriptscriptfont3=\tenex
 \textfont\itfam=\tenit	\def\it{\fam\itfam\tenit}
 \textfont\slfam=\tensl \def\sl{\fam\slfam\tensl}
 \textfont\ttfam=\tentt \def\tt{\fam\ttfam\tentt}
 \textfont\bffam=\tenbf \def\bf{\fam\bffam\tenbf}
 \scriptfont\bffam\sevenbf \scriptscriptfont\bffam=\fivebf
 \tt \ttglue=.5em plus.25em minus.15em
 \normalbaselineskip=12pt
 \setbox\strutbox=\hbox{\vrule height8.5pt depth3.5pt width0pt}
 \let\sc=\eightrm \normalbaselines\rm

\def\eightpoint{\def\rm{\fam0\eightrm}% switch to 8-point type (p415)
 \textfont0=\eightrm \scriptfont0=\sixrm \scriptscriptfont0=\fiverm
 \textfont1=\eighti  \scriptfont1=\sixi  \scriptscriptfont1=\fivei
 \textfont2=\eightsy \scriptfont2=\sixsy \scriptscriptfont2=\fivesy
 \textfont3=\tenex   \scriptfont3=\tenex \scriptscriptfont3=\tenex
 \textfont\itfam=\eightit  \def\it{\fam\itfam\eightit}
 \textfont\slfam=\eightsl  \def\sl{\fam\slfam\eightsl}
 \textfont\ttfam=\eighttt  \def\tt{\fam\ttfam\eighttt}
 \textfont\bffam=\eightbf  \scriptfont\bffam\sixbf
 \scriptscriptfont\bffam=\fivebf  \def\bf{\fam\bffam\eightbf}
 \tt \ttglue=.5em plus.25em minus.15em
 \normalbaselineskip=11pt
 \setbox\strutbox=\hbox{\vrule height7pt depth2pt width0pt}
 \let\sc=\sixrm \normalbaselines\rm}

 \def\simlt{\mathrel{\hbox to 0pt{\lower 3.5pt\hbox{$\mathchar"218$}\hss}
   \raise 1.5pt\hbox{$\mathchar"13C$}}}
 \def\simgt{\mathrel{\hbox to 0pt{\lower 3.5pt\hbox{$\mathchar"218$}\hss}
   \raise 1.5pt\hbox{$\mathchar"13E$}}}
 \def\ref{\par\noindent\parskip=0pt\hangindent12pt\hangafter1}
 \def\reference{\par\noindent\parskip=0pt\hangindent12pt\hangafter1}

 \vsize=53pc
 \hsize=7.0in
 \hoffset=-0.2truein
 \parskip=0pt
 \parindent=12pt
 \baselineskip=12pt
 \lineskip=-12pt
 \lineskiplimit=-24pt
 \pretolerance=100
 \tolerance=1000
 \relpenalty=50
 \vbadness=10000
 \hbadness=10000
 \predisplaypenalty=50
 \postdisplaypenalty=50 
 \topskip=12pt
 \splittopskip=\topskip
 \maxdepth=4pt
 \splitmaxdepth=\maxdepth

 \abovedisplayskip=12pt
 \belowdisplayskip=12pt
 \abovedisplayshortskip=0pt
 \belowdisplayshortskip=12pt

 \def\journal#1{\null\vskip-12pt
   \noindent {\eightrm T{\sixrm HE} A{\sixrm STROPHYSICAL} J{\sixrm OURNAL}
   {\eightrm #1}}
   \vskip-12pt}
 \def\title#1{\null
   \vskip48pt
   \centerline{\twelverm #1}
   \vskip12pt}
 \def\titlem#1{\vskip-6pt
   \centerline{\twelverm #1}
   \vskip6pt}
 \def\author#1{
   \centerline{#1}}
 \def\address#1{
   \centerline{\eightrm #1}}
 \def\date#1#2{
   \centerline {\eightsl Received #1; accepted #2}}
 \def\abstract{
   \vskip18pt
   \centerline{ABSTRACT}
   \vskip10pt
   \par\parshape=1 0.5truein 6.0truein}
 \def\abstractmore{
   \par\parshape=1 0.5truein 6.0truein}
 \def\subject{
   \vskip2pt
   \par\parshape=1 0.5truein 6.0truein
   \noindent
   {\it Subject headings: } }
 \def\maintext{
   \vskip24pt\begindoublecolumns\vskip-12pt}
 \def\section#1{
   \vskip18pt
   \centerline{#1}
   \vskip6pt}
 \def\subsection#1{
   \vskip18pt
   \centerline{#1}
   \vskip6pt}
 \def\subsubsection#1{
   \vskip18pt
   \centerline{{\it{#1}}}
   \vskip6pt}
 \def\refsec#1{\enddoublecolumns
   \vskip24pt
   \centerline{#1}
   \vskip12pt
   \begindoublecolumns
   \baselineskip=11pt plus 1.5pt minus 1pt}

\def\fdg{\hbox{$.\!\!^\circ$}}
\def\arcmin{\hbox{$^\prime$}}
\def\micron{\hbox{$\mu$m}}
\def\arcdeg{\hbox{$^\circ$}}
\def\lesssim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$<$}}}}
\def\gtrsim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$>$}}}}

 \newdimen\h@size
 \h@size=\hsize

 \def\figtop#1#2#3{\topinsert\null\vskip-12pt
  \psfig{file={#1},width=\h@size,silent=yes}
  \vskip-6pt
  \edef\h@old{\the\hsize}\hsize=\h@size
  Fig.~{#2}.---{#3}\vskip12pt\vskip-5.23433pt
  \hsize=\h@old\endinsert\vfuzz=0.5pt}
 \def\tabtitle#1#2{\vskip15pt
   \centerline {TABLE {#1}}\vskip4pt
   \centerline {#2}
   \tabskip=0.5em plus 10.0em minus 0.5em
   \halign to \hsize}
 \def\tabbot#1#2{\null\vskip-24pt
   \edef\h@old{\the\hsize}\hsize=\h@size
   \vskip15pt
   \centerline {{\tenrm TABLE} {\tenrm{#1}}}\vskip4pt
   \centerline {\tenrm{#2}}
   \tabskip=0.5em plus 10.0em minus 0.5em
   \halign to \hsize}
 \def\tabhead#1{
   \noalign{\vskip10pt\hrule\vskip2pt\hrule\vskip6pt}#1}
 \def\tabbody#1{\noalign{\vskip6pt\hrule\vskip6pt}
   #1\noalign{\vskip6pt\hrule\vskip8pt}}
 \def\tabnote#1{\noindent{#1}\vskip17pt
   \vskip-36pt\hsize=\h@old\vfuzz=0.5pt}

 \def\footnoterule{\null}

 \def\JHU{Department of Physics and Astronomy,
   The Johns Hopkins Univeristy,
   Baltimore, MD 21218}
 \def\STScI{Space Telescope Science Institute,
   3700 San Martin Drive,
   Baltimore, MD 21218}

%
% AUTO-EQUATION NUMBER
%
\newcount\Chno\newcount\Eqno\newcount\Eqlt
\def\nxtChno{\global\advance\Chno by 1 \global\Eqno=0 \global\Eqlt=`a}
\def\nxtEqno{\global\advance\Eqno by 1 \global\Eqlt=`a}
\def\nxtEqlt{\global\advance\Eqlt by 1}
\def\ChEq{\the\Eqno}
\def\ChEql{\ChEq\char\the\Eqlt}
\def\Eq{\nxtEqno\eqno(\ChEq)}
\def\EqL{\nxtEqno\eqno(\ChEql)}
\def\Eql{\nxtEqlt\eqno(\ChEql)}
\def\Eqby#1{\nxtEqno\eqno(\ChEq)\xdef#1{\ChEq}}
\def\EqLby#1{\nxtEqno\eqno(\ChEql)\xdef#1{\ChEql}}
\def\Eqlby#1{\nxtEqlt\eqno(\ChEql)\xdef#1{\ChEql}}

%
% psfig.tex
%
% Psfig/TeX 
\def\PsfigVersion{1.9}
% dvips version
%
% All psfig/tex software, documentation, and related files
% in this distribution of psfig/tex are 
% Copyright 1987, 1988, 1991 Trevor J. Darrell
%
% Permission is granted for use and non-profit distribution of psfig/tex 
% providing that this notice is clearly maintained. The right to
% distribute any portion of psfig/tex for profit or as part of any commercial
% product is specifically reserved for the author(s) of that portion.
%
% *** Feel free to make local modifications of psfig as you wish,
% *** but DO NOT post any changed or modified versions of ``psfig''
% *** directly to the net. Send them to me and I'll try to incorporate
% *** them into future versions. If you want to take the psfig code 
% *** and make a new program (subject to the copyright above), distribute it, 
% *** (and maintain it) that's fine, just don't call it psfig.
%
% Bugs and improvements to trevor@media.mit.edu.
%
% Thanks to Greg Hager (GDH) and Ned Batchelder for their contributions
% to the original version of this project.
%
% Modified by J. Daniel Smith on 9 October 1990 to accept the
% %%BoundingBox: comment with or without a space after the colon.  Stole
% file reading code from Tom Rokicki's EPSF.TEX file (see below).
%
% More modifications by J. Daniel Smith on 29 March 1991 to allow the
% the included PostScript figure to be rotated.  The amount of
% rotation is specified by the "angle=" parameter of the \psfig command.
%
% Modified by Robert Russell on June 25, 1991 to allow users to specify
% .ps filenames which don't yet exist, provided they explicitly provide
% boundingbox information via the \psfig command. Note: This will only work
% if the "file=" parameter follows all four "bb???=" parameters in the
% command. This is due to the order in which psfig interprets these params.
%
%  3 Jul 1991	JDS	check if file already read in once
%  4 Sep 1991	JDS	fixed incorrect computation of rotated
%			bounding box
% 25 Sep 1991	GVR	expanded synopsis of \psfig
% 14 Oct 1991	JDS	\fbox code from LaTeX so \psdraft works with TeX
%			changed \typeout to \ps@typeout
% 17 Oct 1991	JDS	added \psscalefirst and \psrotatefirst
%

% From: gvr@cs.brown.edu (George V. Reilly)
%
% \psdraft	draws an outline box, but doesn't include the figure
%		in the DVI file.  Useful for previewing.
%
% \psfull	includes the figure in the DVI file (default).
%
% \psscalefirst width= or height= specifies the size of the figure
% 		before rotation.
% \psrotatefirst (default) width= or height= specifies the size of the
% 		 figure after rotation.  Asymetric figures will
% 		 appear to shrink.
%
% \psfigurepath#1	sets the path to search for the figure
%
% \psfig
% usage: \psfig{file=, figure=, height=, width=,
%			bbllx=, bblly=, bburx=, bbury=,
%			rheight=, rwidth=, clip=, angle=, silent=}
%
%	"file" is the filename.  If no path name is specified and the
%		file is not found in the current directory,
%		it will be looked for in directory \psfigurepath.
%	"figure" is a synonym for "file".
%	By default, the width and height of the figure are taken from
%		the BoundingBox of the figure.
%	If "width" is specified, the figure is scaled so that it has
%		the specified width.  Its height changes proportionately.
%	If "height" is specified, the figure is scaled so that it has
%		the specified height.  Its width changes proportionately.
%	If both "width" and "height" are specified, the figure is scaled
%		anamorphically.
%	"bbllx", "bblly", "bburx", and "bbury" control the PostScript
%		BoundingBox.  If these four values are specified
%               *before* the "file" option, the PSFIG will not try to
%               open the PostScript file.
%	"rheight" and "rwidth" are the reserved height and width
%		of the figure, i.e., how big TeX actually thinks
%		the figure is.  They default to "width" and "height".
%	The "clip" option ensures that no portion of the figure will
%		appear outside its BoundingBox.  "clip=" is a switch and
%		takes no value, but the `=' must be present.
%	The "angle" option specifies the angle of rotation (degrees, ccw).
%	The "silent" option makes \psfig work silently.
%

% check to see if macros already loaded in (maybe some other file says
% "\input psfig") ...
\ifx\undefined\psfig\else\endinput\fi

%
% from a suggestion by eijkhout@csrd.uiuc.edu to allow
% loading as a style file. Changed to avoid problems
% with amstex per suggestion by jbence@math.ucla.edu

\let\LaTeXAtSign=\@
\let\@=\relax
\edef\psfigRestoreAt{\catcode`\@=\number\catcode`@\relax}
%\edef\psfigRestoreAt{\catcode`@=\number\catcode`@\relax}
\catcode`\@=11\relax
\newwrite\@unused
\def\ps@typeout#1{{\let\protect\string\immediate\write\@unused{#1}}}
\ps@typeout{psfig/tex \PsfigVersion}

%% Here's how you define your figure path.  Should be set up with null
%% default and a user useable definition.

\def\figurepath{./}
\def\psfigurepath#1{\edef\figurepath{#1}}

%
% @psdo control structure -- similar to Latex @for.
% I redefined these with different names so that psfig can
% be used with TeX as well as LaTeX, and so that it will not 
% be vunerable to future changes in LaTeX's internal
% control structure,
%
\def\@nnil{\@nil}
\def\@empty{}
\def\@psdonoop#1\@@#2#3{}
\def\@psdo#1:=#2\do#3{\edef\@psdotmp{#2}\ifx\@psdotmp\@empty \else
    \expandafter\@psdoloop#2,\@nil,\@nil\@@#1{#3}\fi}
\def\@psdoloop#1,#2,#3\@@#4#5{\def#4{#1}\ifx #4\@nnil \else
       #5\def#4{#2}\ifx #4\@nnil \else#5\@ipsdoloop #3\@@#4{#5}\fi\fi}
\def\@ipsdoloop#1,#2\@@#3#4{\def#3{#1}\ifx #3\@nnil 
       \let\@nextwhile=\@psdonoop \else
      #4\relax\let\@nextwhile=\@ipsdoloop\fi\@nextwhile#2\@@#3{#4}}
\def\@tpsdo#1:=#2\do#3{\xdef\@psdotmp{#2}\ifx\@psdotmp\@empty \else
    \@tpsdoloop#2\@nil\@nil\@@#1{#3}\fi}
\def\@tpsdoloop#1#2\@@#3#4{\def#3{#1}\ifx #3\@nnil 
       \let\@nextwhile=\@psdonoop \else
      #4\relax\let\@nextwhile=\@tpsdoloop\fi\@nextwhile#2\@@#3{#4}}
% 
% \fbox is defined in latex.tex; so if \fbox is undefined, assume that
% we are not in LaTeX.
% Perhaps this could be done better???
\ifx\undefined\fbox
% \fbox code from modified slightly from LaTeX
\newdimen\fboxrule
\newdimen\fboxsep
\newdimen\ps@tempdima
\newbox\ps@tempboxa
\fboxsep = 3pt
\fboxrule = .4pt
\long\def\fbox#1{\leavevmode\setbox\ps@tempboxa\hbox{#1}\ps@tempdima\fboxrule
    \advance\ps@tempdima \fboxsep \advance\ps@tempdima \dp\ps@tempboxa
   \hbox{\lower \ps@tempdima\hbox
  {\vbox{\hrule height \fboxrule
          \hbox{\vrule width \fboxrule \hskip\fboxsep
          \vbox{\vskip\fboxsep \box\ps@tempboxa\vskip\fboxsep}\hskip 
                 \fboxsep\vrule width \fboxrule}
                 \hrule height \fboxrule}}}}
\fi
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% file reading stuff from epsf.tex
%   EPSF.TEX macro file:
%   Written by Tomas Rokicki of Radical Eye Software, 29 Mar 1989.
%   Revised by Don Knuth, 3 Jan 1990.
%   Revised by Tomas Rokicki to accept bounding boxes with no
%      space after the colon, 18 Jul 1990.
%   Portions modified/removed for use in PSFIG package by
%      J. Daniel Smith, 9 October 1990.
%
\newread\ps@stream
\newif\ifnot@eof       % continue looking for the bounding box?
\newif\if@noisy        % report what you're making?
\newif\if@atend        % %%BoundingBox: has (at end) specification
\newif\if@psfile       % does this look like a PostScript file?
%
% PostScript files should start with `%!'
%
{\catcode`\%=12\global\gdef\epsf@start{%!}}
\def\epsf@PS{PS}
%
\def\epsf@getbb#1{%
%
%   The first thing we need to do is to open the
%   PostScript file, if possible.
%
\openin\ps@stream=#1
\ifeof\ps@stream\ps@typeout{Error, File #1 not found}\else
%
%   Okay, we got it. Now we'll scan lines until we find one that doesn't
%   start with %. We're looking for the bounding box comment.
%
   {\not@eoftrue \chardef\other=12
    \def\do##1{\catcode`##1=\other}\dospecials \catcode`\ =10
    \loop
       \if@psfile
	  \read\ps@stream to \epsf@fileline
       \else{
	  \obeyspaces
          \read\ps@stream to \epsf@tmp\global\let\epsf@fileline\epsf@tmp}
       \fi
       \ifeof\ps@stream\not@eoffalse\else
%
%   Check the first line for `%!'.  Issue a warning message if its not
%   there, since the file might not be a PostScript file.
%
       \if@psfile\else
       \expandafter\epsf@test\epsf@fileline:. \\%
       \fi
%
%   We check to see if the first character is a % sign;
%   if so, we look further and stop only if the line begins with
%   `%%BoundingBox:' and the `(atend)' specification was not found.
%   That is, the only way to stop is when the end of file is reached,
%   or a `%%BoundingBox: llx lly urx ury' line is found.
%
          \expandafter\epsf@aux\epsf@fileline:. \\%
       \fi
   \ifnot@eof\repeat
   }\closein\ps@stream\fi}%
%
% This tests if the file we are reading looks like a PostScript file.
%
\long\def\epsf@test#1#2#3:#4\\{\def\epsf@testit{#1#2}
			\ifx\epsf@testit\epsf@start\else
\ps@typeout{Warning! File does not start with `\epsf@start'.  It may not be a PostScript file.}
			\fi
			\@psfiletrue} % don't test after 1st line
%
%   We still need to define the tricky \epsf@aux macro. This requires
%   a couple of magic constants for comparison purposes.
%
{\catcode`\%=12\global\let\epsf@percent=%\global\def\epsf@bblit{%BoundingBox}}
%
%
%   So we're ready to check for `%BoundingBox:' and to grab the
%   values if they are found.  We continue searching if `(at end)'
%   was found after the `%BoundingBox:'.
%
\long\def\epsf@aux#1#2:#3\\{\ifx#1\epsf@percent
   \def\epsf@testit{#2}\ifx\epsf@testit\epsf@bblit
	\@atendfalse
        \epsf@atend #3 . \\%
	\if@atend	
	   \if@verbose{
		\ps@typeout{psfig: found `(atend)'; continuing search}
	   }\fi
        \else
        \epsf@grab #3 . . . \\%
        \not@eoffalse
        \global\no@bbfalse
        \fi
   \fi\fi}%
%
%   Here we grab the values and stuff them in the appropriate definitions.
%
\def\epsf@grab #1 #2 #3 #4 #5\\{%
   \global\def\epsf@llx{#1}\ifx\epsf@llx\empty
      \epsf@grab #2 #3 #4 #5 .\\\else
   \global\def\epsf@lly{#2}%
   \global\def\epsf@urx{#3}\global\def\epsf@ury{#4}\fi}%
%
% Determine if the stuff following the %%BoundingBox is `(atend)'
% J. Daniel Smith.  Copied from \epsf@grab above.
%
\def\epsf@atendlit{(atend)} 
\def\epsf@atend #1 #2 #3\\{%
   \def\epsf@tmp{#1}\ifx\epsf@tmp\empty
      \epsf@atend #2 #3 .\\\else
   \ifx\epsf@tmp\epsf@atendlit\@atendtrue\fi\fi}


% End of file reading stuff from epsf.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% trigonometry stuff from "trig.tex"
\chardef\psletter = 11 % won't conflict with \begin{letter} now...
\chardef\other = 12

\newif \ifdebug %%% turn me on to see TeX hard at work ...
\newif\ifc@mpute %%% don't need to compute some values
\c@mputetrue % but assume that we do

\let\then = \relax
\def\r@dian{pt }
\let\r@dians = \r@dian
\let\dimensionless@nit = \r@dian
\let\dimensionless@nits = \dimensionless@nit
\def\internal@nit{sp }
\let\internal@nits = \internal@nit
\newif\ifstillc@nverging
\def \Mess@ge #1{\ifdebug \then \message {#1} \fi}

{ %%% Things that need abnormal catcodes %%%
	\catcode `\@ = \psletter
	\gdef \nodimen {\expandafter \n@dimen \the \dimen}
	\gdef \term #1 #2 #3%
	       {\edef \t@ {\the #1}%%% freeze parameter 1 (count, by value)
		\edef \t@@ {\expandafter \n@dimen \the #2\r@dian}%
				   %%% freeze parameter 2 (dimen, by value)
		\t@rm {\t@} {\t@@} {#3}%
	       }
	\gdef \t@rm #1 #2 #3%
	       {{%
		\count 0 = 0
		\dimen 0 = 1 \dimensionless@nit
		\dimen 2 = #2\relax
		\Mess@ge {Calculating term #1 of \nodimen 2}%
		\loop
		\ifnum	\count 0 < #1
		\then	\advance \count 0 by 1
			\Mess@ge {Iteration \the \count 0 \space}%
			\Multiply \dimen 0 by {\dimen 2}%
			\Mess@ge {After multiplication, term = \nodimen 0}%
			\Divide \dimen 0 by {\count 0}%
			\Mess@ge {After division, term = \nodimen 0}%
		\repeat
		\Mess@ge {Final value for term #1 of 
				\nodimen 2 \space is \nodimen 0}%
		\xdef \Term {#3 = \nodimen 0 \r@dians}%
		\aftergroup \Term
	       }}
	\catcode `\p = \other
	\catcode `\t = \other
	\gdef \n@dimen #1pt{#1} %%% throw away the ``pt''
}

\def \Divide #1by #2{\divide #1 by #2} %%% just a synonym

\def \Multiply #1by #2%%% allows division of a dimen by a dimen
       {{%%% should really freeze parameter 2 (dimen, passed by value)
	\count 0 = #1\relax
	\count 2 = #2\relax
	\count 4 = 65536
	\Mess@ge {Before scaling, count 0 = \the \count 0 \space and
			count 2 = \the \count 2}%
	\ifnum	\count 0 > 32767 %%% do our best to avoid overflow
	\then	\divide \count 0 by 4
		\divide \count 4 by 4
	\else	\ifnum	\count 0 < -32767
		\then	\divide \count 0 by 4
			\divide \count 4 by 4
		\else
		\fi
	\fi
	\ifnum	\count 2 > 32767 %%% while retaining reasonable accuracy
	\then	\divide \count 2 by 4
		\divide \count 4 by 4
	\else	\ifnum	\count 2 < -32767
		\then	\divide \count 2 by 4
			\divide \count 4 by 4
		\else
		\fi
	\fi
	\multiply \count 0 by \count 2
	\divide \count 0 by \count 4
	\xdef \product {#1 = \the \count 0 \internal@nits}%
	\aftergroup \product
       }}

\def\r@duce{\ifdim\dimen0 > 90\r@dian \then   % sin(x+90) = sin(180-x)
		\multiply\dimen0 by -1
		\advance\dimen0 by 180\r@dian
		\r@duce
	    \else \ifdim\dimen0 < -90\r@dian \then  % sin(-x) = sin(360+x)
		\advance\dimen0 by 360\r@dian
		\r@duce
		\fi
	    \fi}

\def\Sine#1%
       {{%
	\dimen 0 = #1 \r@dian
	\r@duce
	\ifdim\dimen0 = -90\r@dian \then
	   \dimen4 = -1\r@dian
	   \c@mputefalse
	\fi
	\ifdim\dimen0 = 90\r@dian \then
	   \dimen4 = 1\r@dian
	   \c@mputefalse
	\fi
	\ifdim\dimen0 = 0\r@dian \then
	   \dimen4 = 0\r@dian
	   \c@mputefalse
	\fi
%
	\ifc@mpute \then
        	% convert degrees to radians
		\divide\dimen0 by 180
		\dimen0=3.141592654\dimen0
%
		\dimen 2 = 3.1415926535897963\r@dian %%% a well-known constant
		\divide\dimen 2 by 2 %%% we only deal with -pi/2 : pi/2
		\Mess@ge {Sin: calculating Sin of \nodimen 0}%
		\count 0 = 1 %%% see power-series expansion for sine
		\dimen 2 = 1 \r@dian %%% ditto
		\dimen 4 = 0 \r@dian %%% ditto
		\loop
			\ifnum	\dimen 2 = 0 %%% then we've done
			\then	\stillc@nvergingfalse 
			\else	\stillc@nvergingtrue
			\fi
			\ifstillc@nverging %%% then calculate next term
			\then	\term {\count 0} {\dimen 0} {\dimen 2}%
				\advance \count 0 by 2
				\count 2 = \count 0
				\divide \count 2 by 2
				\ifodd	\count 2 %%% signs alternate
				\then	\advance \dimen 4 by \dimen 2
				\else	\advance \dimen 4 by -\dimen 2
				\fi
		\repeat
	\fi		
			\xdef \sine {\nodimen 4}%
       }}

% Now the Cosine can be calculated easily by calling \Sine
\def\Cosine#1{\ifx\sine\UnDefined\edef\Savesine{\relax}\else
		             \edef\Savesine{\sine}\fi
	{\dimen0=#1\r@dian\advance\dimen0 by 90\r@dian
	 \Sine{\nodimen 0}
	 \xdef\cosine{\sine}
	 \xdef\sine{\Savesine}}}	      
% end of trig stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\psdraft{
	\def\@psdraft{0}
	%\ps@typeout{draft level now is \@psdraft \space . }
}
\def\psfull{
	\def\@psdraft{100}
	%\ps@typeout{draft level now is \@psdraft \space . }
}

\psfull

\newif\if@scalefirst
\def\psscalefirst{\@scalefirsttrue}
\def\psrotatefirst{\@scalefirstfalse}
\psrotatefirst

\newif\if@draftbox
\def\psnodraftbox{
	\@draftboxfalse
}
\def\psdraftbox{
	\@draftboxtrue
}
\@draftboxtrue

\newif\if@prologfile
\newif\if@postlogfile
\def\pssilent{
	\@noisyfalse
}
\def\psnoisy{
	\@noisytrue
}
\psnoisy
%%% These are for the option list.
%%% A specification of the form a = b maps to calling \@p@@sa{b}
\newif\if@bbllx
\newif\if@bblly
\newif\if@bburx
\newif\if@bbury
\newif\if@height
\newif\if@width
\newif\if@rheight
\newif\if@rwidth
\newif\if@angle
\newif\if@clip
\newif\if@verbose
\def\@p@@sclip#1{\@cliptrue}


\newif\if@decmpr

%%% GDH 7/26/87 -- changed so that it first looks in the local directory,
%%% then in a specified global directory for the ps file.
%%% RPR 6/25/91 -- changed so that it defaults to user-supplied name if
%%% boundingbox info is specified, assuming graphic will be created by
%%% print time.
%%% TJD 10/19/91 -- added bbfile vs. file distinction, and @decmpr flag

\def\@p@@sfigure#1{\def\@p@sfile{null}\def\@p@sbbfile{null}
	        \openin1=#1.bb
		\ifeof1\closein1
	        	\openin1=\figurepath#1.bb
			\ifeof1\closein1
			        \openin1=#1
				\ifeof1\closein1%
				       \openin1=\figurepath#1
					\ifeof1
					   \ps@typeout{Error, File #1 not found}
						\if@bbllx\if@bblly
				   		\if@bburx\if@bbury
			      				\def\@p@sfile{#1}%
			      				\def\@p@sbbfile{#1}%
							\@decmprfalse
				  	   	\fi\fi\fi\fi
					\else\closein1
				    		\def\@p@sfile{\figurepath#1}%
				    		\def\@p@sbbfile{\figurepath#1}%
						\@decmprfalse
	                       		\fi%
			 	\else\closein1%
					\def\@p@sfile{#1}
					\def\@p@sbbfile{#1}
					\@decmprfalse
			 	\fi
			\else
				\def\@p@sfile{\figurepath#1}
				\def\@p@sbbfile{\figurepath#1.bb}
				\@decmprtrue
			\fi
		\else
			\def\@p@sfile{#1}
			\def\@p@sbbfile{#1.bb}
			\@decmprtrue
		\fi}

\def\@p@@sfile#1{\@p@@sfigure{#1}}

\def\@p@@sbbllx#1{
		%\ps@typeout{bbllx is #1}
		\@bbllxtrue
		\dimen100=#1
		\edef\@p@sbbllx{\number\dimen100}
}
\def\@p@@sbblly#1{
		%\ps@typeout{bblly is #1}
		\@bbllytrue
		\dimen100=#1
		\edef\@p@sbblly{\number\dimen100}
}
\def\@p@@sbburx#1{
		%\ps@typeout{bburx is #1}
		\@bburxtrue
		\dimen100=#1
		\edef\@p@sbburx{\number\dimen100}
}
\def\@p@@sbbury#1{
		%\ps@typeout{bbury is #1}
		\@bburytrue
		\dimen100=#1
		\edef\@p@sbbury{\number\dimen100}
}
\def\@p@@sheight#1{
		\@heighttrue
		\dimen100=#1
   		\edef\@p@sheight{\number\dimen100}
		%\ps@typeout{Height is \@p@sheight}
}
\def\@p@@swidth#1{
		%\ps@typeout{Width is #1}
		\@widthtrue
		\dimen100=#1
		\edef\@p@swidth{\number\dimen100}
}
\def\@p@@srheight#1{
		%\ps@typeout{Reserved height is #1}
		\@rheighttrue
		\dimen100=#1
		\edef\@p@srheight{\number\dimen100}
}
\def\@p@@srwidth#1{
		%\ps@typeout{Reserved width is #1}
		\@rwidthtrue
		\dimen100=#1
		\edef\@p@srwidth{\number\dimen100}
}
\def\@p@@sangle#1{
		%\ps@typeout{Rotation is #1}
		\@angletrue
%		\dimen100=#1
		\edef\@p@sangle{#1} %\number\dimen100}
}
\def\@p@@ssilent#1{ 
		\@verbosefalse
}
\def\@p@@sprolog#1{\@prologfiletrue\def\@prologfileval{#1}}
\def\@p@@spostlog#1{\@postlogfiletrue\def\@postlogfileval{#1}}
\def\@cs@name#1{\csname #1\endcsname}
\def\@setparms#1=#2,{\@cs@name{@p@@s#1}{#2}}
%
% initialize the defaults (size the size of the figure)
%
\def\ps@init@parms{
		\@bbllxfalse \@bbllyfalse
		\@bburxfalse \@bburyfalse
		\@heightfalse \@widthfalse
		\@rheightfalse \@rwidthfalse
		\def\@p@sbbllx{}\def\@p@sbblly{}
		\def\@p@sbburx{}\def\@p@sbbury{}
		\def\@p@sheight{}\def\@p@swidth{}
		\def\@p@srheight{}\def\@p@srwidth{}
		\def\@p@sangle{0}
		\def\@p@sfile{} \def\@p@sbbfile{}
		\def\@p@scost{10}
		\def\@sc{}
		\@prologfilefalse
		\@postlogfilefalse
		\@clipfalse
		\if@noisy
			\@verbosetrue
		\else
			\@verbosefalse
		\fi
}
%
% Go through the options setting things up.
%
\def\parse@ps@parms#1{
	 	\@psdo\@psfiga:=#1\do
		   {\expandafter\@setparms\@psfiga,}}
%
% Compute bb height and width
%
\newif\ifno@bb
\def\bb@missing{
	\if@verbose{
		\ps@typeout{psfig: searching \@p@sbbfile \space  for bounding box}
	}\fi
	\no@bbtrue
	\epsf@getbb{\@p@sbbfile}
        \ifno@bb \else \bb@cull\epsf@llx\epsf@lly\epsf@urx\epsf@ury\fi
}	
\def\bb@cull#1#2#3#4{
	\dimen100=#1 bp\edef\@p@sbbllx{\number\dimen100}
	\dimen100=#2 bp\edef\@p@sbblly{\number\dimen100}
	\dimen100=#3 bp\edef\@p@sbburx{\number\dimen100}
	\dimen100=#4 bp\edef\@p@sbbury{\number\dimen100}
	\no@bbfalse
}
% rotate point (#1,#2) about (0,0).
% The sine and cosine of the angle are already stored in \sine and
% \cosine.  The result is placed in (\p@intvaluex, \p@intvaluey).
\newdimen\p@intvaluex
\newdimen\p@intvaluey
\def\rotate@#1#2{{\dimen0=#1 sp\dimen1=#2 sp
%            	calculate x' = x \cos\theta - y \sin\theta
		  \global\p@intvaluex=\cosine\dimen0
		  \dimen3=\sine\dimen1
		  \global\advance\p@intvaluex by -\dimen3
% 		calculate y' = x \sin\theta + y \cos\theta
		  \global\p@intvaluey=\sine\dimen0
		  \dimen3=\cosine\dimen1
		  \global\advance\p@intvaluey by \dimen3
		  }}
\def\compute@bb{
		\no@bbfalse
		\if@bbllx \else \no@bbtrue \fi
		\if@bblly \else \no@bbtrue \fi
		\if@bburx \else \no@bbtrue \fi
		\if@bbury \else \no@bbtrue \fi
		\ifno@bb \bb@missing \fi
		\ifno@bb \ps@typeout{FATAL ERROR: no bb supplied or found}
			\no-bb-error
		\fi
		%
%\ps@typeout{BB: \@p@sbbllx, \@p@sbblly, \@p@sbburx, \@p@sbbury} 
%
% store height/width of original (unrotated) bounding box
		\count203=\@p@sbburx
		\count204=\@p@sbbury
		\advance\count203 by -\@p@sbbllx
		\advance\count204 by -\@p@sbblly
		\edef\ps@bbw{\number\count203}
		\edef\ps@bbh{\number\count204}
		%\ps@typeout{ psbbh = \ps@bbh, psbbw = \ps@bbw }
		\if@angle 
			\Sine{\@p@sangle}\Cosine{\@p@sangle}
	        	{\dimen100=\maxdimen\xdef\r@p@sbbllx{\number\dimen100}
					    \xdef\r@p@sbblly{\number\dimen100}
			                    \xdef\r@p@sbburx{-\number\dimen100}
					    \xdef\r@p@sbbury{-\number\dimen100}}
%
% Need to rotate all four points and take the X-Y extremes of the new
% points as the new bounding box.
                        \def\minmaxtest{
			   \ifnum\number\p@intvaluex<\r@p@sbbllx
			      \xdef\r@p@sbbllx{\number\p@intvaluex}\fi
			   \ifnum\number\p@intvaluex>\r@p@sbburx
			      \xdef\r@p@sbburx{\number\p@intvaluex}\fi
			   \ifnum\number\p@intvaluey<\r@p@sbblly
			      \xdef\r@p@sbblly{\number\p@intvaluey}\fi
			   \ifnum\number\p@intvaluey>\r@p@sbbury
			      \xdef\r@p@sbbury{\number\p@intvaluey}\fi
			   }
%			lower left
			\rotate@{\@p@sbbllx}{\@p@sbblly}
			\minmaxtest
%			upper left
			\rotate@{\@p@sbbllx}{\@p@sbbury}
			\minmaxtest
%			lower right
			\rotate@{\@p@sbburx}{\@p@sbblly}
			\minmaxtest
%			upper right
			\rotate@{\@p@sbburx}{\@p@sbbury}
			\minmaxtest
			\edef\@p@sbbllx{\r@p@sbbllx}\edef\@p@sbblly{\r@p@sbblly}
			\edef\@p@sbburx{\r@p@sbburx}\edef\@p@sbbury{\r@p@sbbury}
%\ps@typeout{rotated BB: \r@p@sbbllx, \r@p@sbblly, \r@p@sbburx, \r@p@sbbury}
		\fi
		\count203=\@p@sbburx
		\count204=\@p@sbbury
		\advance\count203 by -\@p@sbbllx
		\advance\count204 by -\@p@sbblly
		\edef\@bbw{\number\count203}
		\edef\@bbh{\number\count204}
		%\ps@typeout{ bbh = \@bbh, bbw = \@bbw }
}
%
% \in@hundreds performs #1 * (#2 / #3) correct to the hundreds,
%	then leaves the result in @result
%
\def\in@hundreds#1#2#3{\count240=#2 \count241=#3
		     \count100=\count240	% 100 is first digit #2/#3
		     \divide\count100 by \count241
		     \count101=\count100
		     \multiply\count101 by \count241
		     \advance\count240 by -\count101
		     \multiply\count240 by 10
		     \count101=\count240	%101 is second digit of #2/#3
		     \divide\count101 by \count241
		     \count102=\count101
		     \multiply\count102 by \count241
		     \advance\count240 by -\count102
		     \multiply\count240 by 10
		     \count102=\count240	% 102 is the third digit
		     \divide\count102 by \count241
		     \count200=#1\count205=0
		     \count201=\count200
			\multiply\count201 by \count100
		 	\advance\count205 by \count201
		     \count201=\count200
			\divide\count201 by 10
			\multiply\count201 by \count101
			\advance\count205 by \count201
			%
		     \count201=\count200
			\divide\count201 by 100
			\multiply\count201 by \count102
			\advance\count205 by \count201
			%
		     \edef\@result{\number\count205}
}
\def\compute@wfromh{
		% computing : width = height * (bbw / bbh)
		\in@hundreds{\@p@sheight}{\@bbw}{\@bbh}
		%\ps@typeout{ \@p@sheight * \@bbw / \@bbh, = \@result }
		\edef\@p@swidth{\@result}
		%\ps@typeout{w from h: width is \@p@swidth}
}
\def\compute@hfromw{
		% computing : height = width * (bbh / bbw)
	        \in@hundreds{\@p@swidth}{\@bbh}{\@bbw}
		%\ps@typeout{ \@p@swidth * \@bbh / \@bbw = \@result }
		\edef\@p@sheight{\@result}
		%\ps@typeout{h from w : height is \@p@sheight}
}
\def\compute@handw{
		\if@height 
			\if@width
			\else
				\compute@wfromh
			\fi
		\else 
			\if@width
				\compute@hfromw
			\else
				\edef\@p@sheight{\@bbh}
				\edef\@p@swidth{\@bbw}
			\fi
		\fi
}
\def\compute@resv{
		\if@rheight \else \edef\@p@srheight{\@p@sheight} \fi
		\if@rwidth \else \edef\@p@srwidth{\@p@swidth} \fi
		%\ps@typeout{rheight = \@p@srheight, rwidth = \@p@srwidth}
}
%		
% Compute any missing values
\def\compute@sizes{
	\compute@bb
	\if@scalefirst\if@angle
% at this point the bounding box has been adjsuted correctly for
% rotation.  PSFIG does all of its scaling using \@bbh and \@bbw.  If
% a width= or height= was specified along with \psscalefirst, then the
% width=/height= value needs to be adjusted to match the new (rotated)
% bounding box size (specifed in \@bbw and \@bbh).
%    \ps@bbw       width=
%    -------  =  ---------- 
%    \@bbw       new width=
% so `new width=' = (width= * \@bbw) / \ps@bbw; where \ps@bbw is the
% width of the original (unrotated) bounding box.
	\if@width
	   \in@hundreds{\@p@swidth}{\@bbw}{\ps@bbw}
	   \edef\@p@swidth{\@result}
	\fi
	\if@height
	   \in@hundreds{\@p@sheight}{\@bbh}{\ps@bbh}
	   \edef\@p@sheight{\@result}
	\fi
	\fi\fi
	\compute@handw
	\compute@resv}

%
% \psfig
% usage : \psfig{file=, height=, width=, bbllx=, bblly=, bburx=, bbury=,
%			rheight=, rwidth=, clip=}
%
% "clip=" is a switch and takes no value, but the `=' must be present.
\def\psfig#1{\vbox {
	% do a zero width hard space so that a single
	% \psfig in a centering enviornment will behave nicely
	%{\setbox0=\hbox{\ }\ \hskip-\wd0}
	%
	\ps@init@parms
	\parse@ps@parms{#1}
	\compute@sizes
	%
	\ifnum\@p@scost<\@psdraft{
		%
		\special{ps::[begin] 	\@p@swidth \space \@p@sheight \space
				\@p@sbbllx \space \@p@sbblly \space
				\@p@sbburx \space \@p@sbbury \space
				startTexFig \space }
		\if@angle
			\special {ps:: \@p@sangle \space rotate \space} 
		\fi
		\if@clip{
			\if@verbose{
				\ps@typeout{(clip)}
			}\fi
			\special{ps:: doclip \space }
		}\fi
		\if@prologfile
		    \special{ps: plotfile \@prologfileval \space } \fi
		\if@decmpr{
			\if@verbose{
				\ps@typeout{psfig: including \@p@sfile.Z \space }
			}\fi
			\special{ps: plotfile "`zcat \@p@sfile.Z" \space }
		}\else{
			\if@verbose{
				\ps@typeout{psfig: including \@p@sfile \space }
			}\fi
			\special{ps: plotfile \@p@sfile \space }
		}\fi
		\if@postlogfile
		    \special{ps: plotfile \@postlogfileval \space } \fi
		\special{ps::[end] endTexFig \space }
		% Create the vbox to reserve the space for the figure.
		\vbox to \@p@srheight sp{
		% 1/92 TJD Changed from "true sp" to "sp" for magnification.
			\hbox to \@p@srwidth sp{
				\hss
			}
		\vss
		}
	}\else{
		% draft figure, just reserve the space and print the
		% path name.
		\if@draftbox{		
			% Verbose draft: print file name in box
			\hbox{\frame{\vbox to \@p@srheight sp{
			\vss
			\hbox to \@p@srwidth sp{ \hss \@p@sfile \hss }
			\vss
			}}}
		}\else{
			% Non-verbose draft
			\vbox to \@p@srheight sp{
			\vss
			\hbox to \@p@srwidth sp{\hss}
			\vss
			}
		}\fi	



	}\fi
}}
\psfigRestoreAt
\let\@=\LaTeXAtSign

%
% dblecols.tex
%
%
% double columns work (hard)
%\check
\edef\catcodeat{\the\catcode`\@}\catcode`\@=11
\newbox\p@artialpage\newbox\r@emainder
\newbox\b@oxzero\newbox\b@oxone\newbox\b@oxtwo\newbox\b@oxthree
\newdimen\c@oldimen
\newdimen\i@nterskip
%
\newdimen\p@ageheight
\newdimen\p@agewidth
\newdimen\p@agework
\newdimen\v@dblesize
%
% pour que \pagetotal et \pagegoal soient initialises... (very dirty trick)
\def\v@oidbox{\hrule height 0pt width 0pt}
\def\b@ottomskip{\vskip 0pt plus 10pt}
\def\dble@safety{0.1}
%
\def\compute@left{\p@agework=\p@ageheight
 \ifvoid\footins\relax\else
   \advance\p@agework by -\ht\footins
   \advance\p@agework by -\skip\footins
 \fi 
 \ifvoid\topins\relax\else
   \advance\p@agework by -\ht\topins
   \advance\p@agework by -\skip\topins
 \fi}%
%
%\check
\def\out@sofar{{\def\pagecontents{\ifvoid\topins\else\unvbox\topins\fi
   \p@agesofar
   \ifvoid\footins\else % footnote info is present
     \vskip\skip\footins
     \footnoterule
     \unvbox\footins
   \fi}\hsize=\p@agewidth\vsize=\p@ageheight
   \givenoutput}}
%\check
%
\def\out@partial{{\def\pagecontents{\ifvoid\topins\else\unvbox\topins\fi
   \unvbox\p@artialpage
   \ifvoid\footins\else % footnote info is present
     \vskip\skip\footins
     \footnoterule
     \unvbox\footins
   \fi}\hsize=\p@agewidth\vsize=\p@ageheight
   \givenoutput}}
%
\def\safe@eject{\vsize=\p@ageheight\pagegoal=4\p@ageheight\eject
  \removelastskip}
%\check
%
\def\begindoublecolumns{\p@ageheight=\vsize\p@agewidth=\hsize
\edef\givenoutput{\the\output}%
\edef\restoretopskip{\noexpand
   \topskip=\the\topskip\noexpand\splittopskip=\the\splittopskip}%
\topskip=\baselineskip\splittopskip=\topskip
\edef\restorebaselineskip{\noexpand\baselineskip=\the\baselineskip
   \noexpand\normallineskip=\the\normallineskip}%
%
% securite : compute available height in \p@agework
 \compute@left
 \advance\p@agework by -2\baselineskip
% if there is a risk, then output 
 \ifdim\pagetotal > \p@agework
   \message{Begindoublecolumns: Pagetotal=\the\pagetotal\ >
   P@agework=\the\p@agework}\relax
   {\splittopskip=\topskip\splitmaxdepth=\maxdepth
   \output{\global\setbox\b@oxone=\vbox{\unvbox255}}\safe@eject
   \global\setbox\p@artialpage=\vsplit\b@oxone to \p@agework}\out@partial
   \unvbox\b@oxone
 \fi
%
 \begingroup\multiply\hyphenpenalty by 2\relax
   \widowpenalty 60\relax
   \clubpenalty 30\relax
   \brokenpenalty 50\relax
   \linepenalty 50\relax
   \output={\global\setbox\p@artialpage=\vbox{\unvbox255}}\relax
   \baselineskip=0pt \normallineskip=0pt    
%   \hrule width 5cm
   \boxmaxdepth=0pt\maxdepth=0pt\relax
   \topskip=0pt\splittopskip=0pt\safe@eject
   \restorebaselineskip
% compute available vertical place in half width into \p@agework   
   \compute@left \advance\p@agework by \p@ageheight % 2\p@ageheight-[inserts]
   \v@oidbox
% compute used vertical place in half width into \c@oldimen    
   \global\c@oldimen=2\ht\p@artialpage
   \global\advance\c@oldimen by -\dble@safety\ht\p@artialpage
   \global\advance\c@oldimen by -\dble@safety\ht\p@artialpage
   \global\advance\c@oldimen by \dble@safety\p@agework
   \v@dblesize=\p@agework
   \advance\v@dblesize by -\c@oldimen
   \ifdim\v@dblesize < \baselineskip
     \message{ P@agework=\the\p@agework, C@oldimen=\the\c@oldimen,
       V@dblesize=\the\v@dblesize}
%     \showthe\v@dblesize
   \fi  
%   
   \output={\doublecolumnout}\hsize=0.48\p@agewidth\vsize=2\p@ageheight
 }% end of \begindoublecolumns
% 
%\check
\def\enddoublecolumns{\removelastskip
 \compute@left\advance\p@agework by \p@ageheight
 \advance\v@dblesize by -2\baselineskip
 \ifdim\pagetotal > \v@dblesize
   \output{\global\setbox\r@emainder=\vbox{\unvbox255}}\safe@eject
   \splittopskip=\topskip\boxmaxdepth=\maxdepth
   \global\setbox255=\vsplit\r@emainder to \v@dblesize
   \doublecolumnout
   \unvbox\r@emainder
 \fi   
 \output={\balancecolumns}\safe@eject
 \endgroup %\leftrule
 \vsize=\p@ageheight
 \v@oidbox
 \pagegoal=2\p@ageheight\penalty 10000\p@agesofar
 \vsize=\p@ageheight
 \v@oidbox\pagegoal=\p@ageheight\par\penalty -2000}%
%
\def\doublecolumnout{\splittopskip=\topskip\splitmaxdepth=\maxdepth
 \vsize=\p@ageheight
 \compute@left
 \advance\p@agework by -\ht\p@artialpage
 \global\c@oldimen=2\p@agework
 \global\setbox\b@oxzero=\vsplit255 to \c@oldimen
 \balanceb@oxzero
 \out@sofar
 \vsize=2\p@ageheight\pagegoal=\vsize
 \unvbox255\restoretopskip
 \vsize=2\p@ageheight\pagegoal=\vsize
 \penalty\outputpenalty
}%
%
\def\p@agesofar{\unvbox\p@artialpage\penalty 10000\relax
 \wd\b@oxzero=\hsize \wd\b@oxtwo=\hsize
 \hbox to \p@agewidth{\vtop{\unvbox\b@oxzero}\hfil\vtop{\unvbox\b@oxtwo}}}
%\check
%
\def\balanceb@oxzero{\global\c@oldimen=\ht\b@oxzero
 \global\advance\c@oldimen by \topskip
 \global\advance\c@oldimen by -\baselineskip
 \global\divide\c@oldimen by 2\relax
 \splittopskip=\topskip\splitmaxdepth=\maxdepth
%
{\vbadness=10000\loop
\global\setbox\b@oxthree=\copy\b@oxzero
\global\setbox\b@oxtwo=\vsplit\b@oxthree to \c@oldimen
\global\setbox\b@oxone=\vbox{\unvbox\b@oxtwo}%
\p@agework=\ht\b@oxthree
\advance\p@agework by -\ht\b@oxone
\ifdim\p@agework > \baselineskip
 \global\advance\c@oldimen by 0.2\p@agework
% \message{ C@oldimen +1:\the\c@oldimen, \the\p@agework}
\repeat}\relax
%
{\vbadness=10000\loop
\global\setbox\b@oxthree=\copy\b@oxzero
\global\setbox\b@oxtwo=\vsplit\b@oxthree to \c@oldimen
\global\setbox\b@oxone=\vbox{\unvbox\b@oxtwo}%
\p@agework=\ht\b@oxthree
\advance\p@agework by -\ht\b@oxone
\ifdim\p@agework < -\baselineskip
 \global\advance\c@oldimen by 0.2\p@agework
% \message{ C@oldimen -1:\the\c@oldimen, \the\p@agework}
\repeat}\relax
%
\p@agework=\ht\b@oxthree
\advance\p@agework by -\ht\b@oxone
\ifdim\p@agework > \baselineskip
  \message{SPLIT: p.\the\count0, P@gework: \the\p@agework}\relax
  \i@nterskip=\baselineskip
  \global\setbox\b@oxtwo=\hbox{\rm W}\advance\i@nterskip by -\ht\b@oxtwo
  \global\setbox\b@oxtwo=\vsplit\b@oxthree to 0.5\p@agework
\else
  \i@nterskip=\topskip
\fi
\global\setbox\b@oxzero=\vbox to \c@oldimen{\unvbox\b@oxone
 \vskip\i@nterskip \unvbox\b@oxtwo\b@ottomskip}%
\global\setbox\b@oxtwo=\vbox to \c@oldimen{\unvbox\b@oxthree\b@ottomskip}%
}%
%
\def\balancecolumns{\global\setbox\b@oxzero=\vbox{\unvbox255}\balanceb@oxzero
}%
%\check
%
\def\leftrule{\removelastskip\par\kern -5pt\hbox{\vrule width 0.49\hsize height 0.4pt
\vrule height 6pt}\medskip}
\def\rightrule{\medskip\rightline{\vrule depth 5.6pt height 0.4pt width 0.4pt
\vrule width 0.49\hsize height 0.4pt depth 0pt}\kern -5pt\par}
\catcode`\@=\catcodeat
%


